Confounder-Dependent Bayesian Mixture Model: Characterizing Heterogeneity of Causal Effects in Air Pollution Epidemiology

Several epidemiological studies have provided evidence that long-term exposure to fine particulate matter (PM2.5) increases mortality risk. Furthermore, some population characteristics (e.g., age, race, and socioeconomic status) might play a crucial role in understanding vulnerability to air pollution. To inform policy, it is necessary to identify groups of the population that are more or less vulnerable to air pollution. In causal inference literature, the Group Average Treatment Effect (GATE) is a distinctive facet of the conditional average treatment effect. This widely employed metric serves to characterize the heterogeneity of a treatment effect based on some population characteristics. In this work, we introduce a novel Confounder-Dependent Bayesian Mixture Model (CDBMM) to characterize causal effect heterogeneity. More specifically, our method leverages the flexibility of the dependent Dirichlet process to model the distribution of the potential outcomes conditionally to the covariates and the treatment levels, thus enabling us to: (i) identify heterogeneous and mutually exclusive population groups defined by similar GATEs in a data-driven way, and (ii) estimate and characterize the causal effects within each of the identified groups. Through simulations, we demonstrate the effectiveness of our method in uncovering key insights about treatment effects heterogeneity. We apply our method to claims data from Medicare enrollees in Texas. We found six mutually exclusive groups where the causal effects of PM2.5 on mortality are heterogeneous.

==> notes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Scott and Dan's comments ---


- evitare di usare positive/negative effects, piuttosto decreasing/increasing mortality effects
- usare formule tipo "looks like ..."

- selective survival: vulnerable people died in great number before they enter in the sample (older than 65)
 -- i.e. poor MEN 
 -- attention for hispanics

"other race" = in California comunità asiatica eterogenea

YELLOW PLOT:
corrisponde alla media dei dati matchati ($93\%$)

RED PLOT:
effect driven by age (big impact of the age)
cumulative effect of vulnerabilities catches up to you 

ORANGE PLOT
ZIPcodes with "young" people
black people that have survived racism
(black people, low income, young)

GREENS PLOT:
("protective effect" ... scott ha usato questo termine, a meno che non abbia capito male)

!!!!
chiarire bene che l'area grigia è la media delle caratteristiche dei Maricair enrolees dei zipcode matchati (NON la popolazione californiana)


% -- Dan's comment in Basecamp chat
another small but important point--California has a large Hispanic population, but this group is notoriously miscoded in medicare data possibly rendering this measure meaningless in your results. A better approach would be to use the RTI race code available for a large number of years in the medicare data, which has much better specificity in identifying hispanic individuals


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- comments for the plots ---

- "dual eligibility" instead S.E.S.
- California map with zip-codes colored by groups



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- general comments  ---

- Effective Sample Size:
  we need large ESS for power
  what the sample needs to detect an effect
--> SPURIOUS correlation

- compute CORR(old people, low income)


There's less than you might imagine on selective survival into Medicare. But there's a ton on survival (or selection or collider) bias more generally. Mayeda et al (2018) is really good and has direct implications for our work. That might be the place to start.
 
Gilsanz et al (2021) is also helpful. They also use simulated data to demonstrate what happens when a cohort study starts later in life (as ours does with Medicare) when exposure effects accumulate over time (as PM likely does) in the presence of time-varying confounding. The paper is primarily about the utility of marginal structural models but has implications for our work. 
 
I'm also throwing in Shaw et al. (2021), which looks at selective survival and gender differences in dementia incidence, mostly because I like it--but also because it has a good discussion on when / where / how selective survival does (and does not!) bias estimates and what to do about it.
 
Hayes-Larson et al (2020) is an example where selective survival does *not* explain a paradoxical inverse relationship between cancer and dementia risk. Not directly relevant to our work, but I include it to show that survival bias isn't always the answer to these types of unexpected relationships. There are also a number of papers exploring the 'obesity paradox' and the possible role of selective survival in it.
 
Jbaily et al (2022) and Liu et al (2021) are on exposure disparities by race / ethnicity and income.
 
Pope III et al (2019) reports higher PM2.5-mortality HRs for racialized groups and low-income groups (separately) in a nationally representative cohort that includes people younger than 65.
 
Let me know if those are helpful. Keep us posted. And enjoy your weekends!

%#############################################################

%################################################################

%   ---- Texas ----

Disparities by income in Houston: \citet{hollingsworth2021health}
Disparities by race and income in excess pollutant emissions: \citet{li2019racial}
Differences by age in Texas: \citet{sohrabi2020burden}
And then beyond that, you can point to literature showing (1) a high proportion of Hispanic residents in TX, e.g., the US Census Bureau should have these stats; (2) exposure disparities showing low income and Hispanic people are exposed to more PM, e.g., Jbaily et al 2022 in Nature; and (3) possible higher HR for PM exposure among Hispanic vs White people \citet{di2017air} and among low income (i.e., Medicaid eligible) vs higher income \citet{yazdi2021long}
